Prediction Factory: automated development and collaborative evaluation of predictive models

In this paper, we present a data science automation system called Prediction Factory. The system uses several key automation algorithms to enable data scientists to rapidly develop predictive models and share them with domain experts. To assess the system's impact, we implemented 3 different interfaces for creating predictive modeling projects: baseline automation, full automation, and optional automation. With a dataset of online grocery shopper behaviors, we divided data scientists among the interfaces to specify prediction problems, learn and evaluate models, and write a report for domain experts to judge whether or not to fund to continue working on. In total, 22 data scientists created 94 reports that were judged 296 times by 26 experts. In a head-to-head trial, reports generated utilizing full data science automation interface reports were funded 57.5% of the time, while the ones that used baseline automation were only funded 42.5% of the time. An intermediate interface which supports optional automation generated reports were funded 58.6% more often compared to the baseline. Full automation and optional automation reports were funded about equally when put head-to-head. These results demonstrate that Prediction Factory has implemented a critical amount of automation to augment the role of data scientists and improve business outcomes.

==> assignments.tex <==
Max 
- keep editing prediction engineering
-Kalyan asks: Can you do something about the segmentation algorithm?
-Kalyan asks: Maybe we should also add dfs
- write the cohort space as he has the most information about it.
- 

Ben
- Shorten elo description (i like the text you wrote, but it's probably too in depth for this paper. i think we should aim to shorten to 3 sentences.)  
- could you finalize, dataset, prediction problem space, method space?
 dataset details, prediction problem space, machine learning method space, calculation of results

Kalyan
- intro
- contributions


TODOs
- final results
- discussion


==> ls.tex <==
\section{Label-Segment-Featurize}\label{general}

 

As we worked through numerous data science problems across domains, we identified several underlying commonalities. In a typical situation, a data scientist building a predictive model will start by working with a written or spoken definition of the \oc the end user is interested in predicting, as well as constraints, such as how far ahead of time the end user wishes to make the prediction (\textit{lead}) or how much data should be used to do so \textit{lag}. Given this information, we divide the workflow, in which raw data is transformed into training examples, into three steps: \textit{Label}, \textit{Segment} and \textit{Featurize}. In the next three subsections, we describe these three steps in detail, along with the methods we have developed for each. 

 


%To build a generalizable framework, we considered a number of potential scenarios and use cases from different domains. These domains include  predictive health maintenance, retail, online clickstream data, and electronic health records. Typically, these domains have different end goals (deployment vs. analysis), as well as different time scales for prediction (predict ahead vs. real-time). Our goal is to develop abstractions and be able to develop methods underneath those abstractions that would be general enough, and to delineate \textit{parameters} and \textit{defaults}\footnote{Ultimately, we may choose to define default values for different parameters to improve usability for end users} such that one framework can serve a wide variety of use cases across diverse domains. In Table~\ref{cf} we enumerate different scenarios we encountered when defining predictive problems. 


 
%\textbf{somewhere this has to go: one is time could be samples, events and absolute time and that all our discussion would be for one entity-instance, and the process is simply repeated for all

\subsection{Label}
The goal of the Label step is to \tr through an entity-instance's data and identify a list of three tuples: $< eid, t_c, l>$, where $eid$ identifies the entity-instance to which the training example belongs, $t_c$ the \co time point (or index) prior to which data can be used for learning the model, and $l$ the category of outcome (in binary cases, "positive" or "negative"). We further break this step down into two substeps: 
\begin{enumerate}
   \itemsep-0.1em
\item defining a \ann and 
  \item traversing the data in search of labels.
\end{enumerate}
%Function design is accomplished by the data scientist, and we describe our search method below. 

%The goal of the first step is to \tr through an entity-instances data and identify a list of three tuples: $< e_{id}, t_c, l>$, where $e_{id}$ identifies the entity-instance for which predictions are sought, $t_c$ the  \co time point (or index) at which the prediction is desired, and $l$ the category of outcome (in binary cases, "positive" or "negative"). We break this step down into two substeps: designing an annotation function and searching and annotating the data. Function design is accomplished by the data scientist, and we describe our search method below. 

%In this step, through an interface user can write an annotation function and by the setting a few parameters, can search through the data for an entity-instance to find all the labeled examples. 
% \begin{table}[htb!]
% \centering
% \begin{tabular}{r|l}
% \hline
% Name &Description\\ \hline
% $O_g$& global offset. \\ %\hline
% $O$ &offset\\ %\hline
% $W_p$ & size of prediction window. \\ %\hline
% $n_w$& number of windows\\ %\hline
% $&Ending time point for a \ls\\ %\hline
% \end{tabular}
% \vspace{2mm}
% \caption{Parameters for search.}
% \label{naming}
% \end{table}

%\begin{wrapfigure}{r}{0.25\textwidth}
%\centering
%\includegraphics[width=\linewidth]{figures/Labeling.pdf}
%\caption{Labeling function}\label{fig:labeling}
%\end{wrapfigure}
\noindent \textbf{Defining a \ann:} A \ann, $L(.)$, contains a user-defined logic that
\begin{itemize}
 \itemsep-0.1em
\item is applied to the the data within the \lw,
\item can optionally use data prior to the \co $t_c$, but must use the data within the \lw, and
  \item produces a \textit{label} the user is interested in predicting.
\end{itemize}
 \begin{figure}%{r}{0.25\textwidth}
\centering
\includegraphics[width=0.85\linewidth]{figures/FeatureReduce.pdf}
\caption{The \textit{feature-reduce} abstraction for defining prediction labels. It works by calculating a feature value for each event/sample in the labeling window. In this example, we are calculating a binary feature at each event (purchase event or not). Then, it reduces that list of features to a single label using a function such as \textsc{any}}
\end{figure}
When we attempted to define labeling functions for a variety of well-known predictive problems over different domains, we realized that they typically share two additional characteristics. First, samples within the window are each transformed into another value, and in almost every case, this value is equivalent to a \textit{feature} in the machine learning sense. Second, an aggregation logic is applied to these values in order to generate the label.

Noting these consistencies, we created a \textit{feature-reduce} abstraction. This abstraction allows data scientists to develop their own labeling functions with the same language they will later use to develop features. Examples of how \textit{feature-reduce} is applied in 3 different problems in 3 different domains can be seen in Table \ref{tab:examples}. 
 
%In the annotation phase, the framework applies one or several user-supplied outcome functions to the data (a time-varying column or a group of columns), and produces a list of three tuple $e_{id}, t_c, l$. Where $e_{id}$ specifies the id of the the entity instance, $t_c$ is defined as the last time point at which the data is allowed to be used for learning, and $l$ is the label. For each entry in the list, we define the first time stamp as the earliest time at which the data can be used. 

%\begin{table}[htb!]
%\centering\normalsize
%\renewcommand{\arraystretch}{1.0}
%\begin{tabularx}{\linewidth}{@{}llA@{}}
%\hline
%Feature & Reduce & Outcome \\ \hline
%??? & ??? & Example \ref{disc} involves an outcome based on an instantaneous, discrete happening. This will evaluate to true whenever the customer under consideration buys the product $i$.\\ 
%??? & ??? & In example \ref{cont1}, the outcome  happens over a window, and can fully become true only at minute 27.  \\\hline
%\end{tabularx}
%\medskip
%\caption{Examples}
%\label{tab:examples}
%\end{table}
%This is illustrated in Figure~\ref{fig:labeling}. We note that this particular abstraction covers a wide range of \anns we came across in different domains. This definition allows users to write a function over a window, without worrying about traversing the data to apply this function and generate labels. Below we present a traversal algorithm that achieves it. 


%\begin{exmp}\label{disc}
%In a database of retail transactions, \textit{did a particular customer buy product $i$?}
%\end{exmp}

%Example \ref{disc} involves an outcome based on an instantaneous, discrete happening. This will evaluate to true whenever the customer under consideration buys the product $i$.

%\begin{exmp}\label{cont1}
%For a given patient's arterial blood pressure time series, evaluate whether his or her blood pressure remained at less than 60mmHg for 27 consecutive minutes within any possible 30-minute window.
%\end{exmp}
%In example \ref{cont1}, the outcome  happens over a window, and can fully become true only at minute 27.  


\input{table3_2}
\noindent \textbf{Traversal algorithm}: Given the \ann, our next goal is to design a traversal algorithm that searches through the data to identify several possible training examples. A simple design of such an algorithm would entail setting $t_c$ at every time point where a data sample is present in the entity-instance's time span, and evaluating the \ann.  
\input{search}
To do this in a tractable way, we propose to iterate over the data samples by specifying the number of $t_c$'s to consider, $n_w$, the spacing between them, $O$, and the size of the \lw, $w_l$. Pseudocode is presented in Algorithm \ref{search}, and the process is illustrated through an example retail dataset in Figure \ref{fig:label_segment}. It is important to note that the traversal algorithm does not make use of any information about the logic inside the \ann. The only information that is shared between it and the \ann is the length of \lw. We imagine that several different and perhaps efficient alternatives are possible for the traversal algorithm. To preserve generalizability, we recommend alternate designs to follow the abstractions for the labeling function, and the inputs and outputs, we suggest for the algorithm. For example, an alternate algorithm can use the size of \lw to skip portions of time series after one instance label is found. While using information from the logic inside the labeling function can aid in an efficient traversal, it could potentially result in a very specific traversal algorithm. 


%\begin{itemize}
   % \item Global offset: This parameter, set in hours, is used to generate the list of $t_c$'s uniformly for all entity instances, starting from midnight of their first time stamp and adding $t_c$ every $O_g$ hours. 
   % 
   % \item Offset: When the offset is specified instead of $O_g$, the first $t_c$ is aligned with the first time stamp for the entity-instance, and subsequent time stamps are $O$ apart. (Note that this does not result in uniform $t_c$'s for all entities.)  
   % \item Prediction window: This parameter sets the time span of data after a particular $t_c$ that the annotation function uses to come up with a label. 
    
    %\item Number of windows: This parameter sets an upper bound on the number of $t_c$'s generated for an entity instance. 
%\end{itemize} 

% \input{table2}

\subsection{Segment}
Given the \textit{lead} and \textit{lag} parameters and the labels, this step identifies segments defined by the four tuples $< eid, t_{start}, t_{stop}, l>$, where $t_{start}$ and $t_{stop}$ represent the time points that will bound the samples used for learning. We call this the ``\textit{learning segment.''} 
%Segmenting entails identifying the \ls for each training example, so they can be passed to the feature engineering step. A learning segment is defined by $t_{start}$, $t_{stop}$, $l$, and $e_{id}$. The first two points, $t_{start}$ and $t_{stop}$, identify start and stop times that define a segment of data that could be used to learn a machine learning model (via. feature engineering and modeling). A segmenting algorithm receives the list of all possible training examples from the \textit{annotation} phase. Next present multiple considerations that determine of how segment and subselect from the annotation examples.



\input{segment}
\noindent \textbf{Lead, Lag, and units} 
\begin{itemize}
\item \textbf{Lead}: For a predictive problem, the $lead$ time specifies how far ahead the user wants to predict the label. For many predictive problems, predicting far ahead (high $lead$) enables value creation, and makes predictive problems interesting. For example, a retailer may want to predict future customer churn as soon as possible. 
\begin{figure*}[htb!]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/label_segment}
    \caption{Figure illustrating the process of traversing, labeling, and segmenting the data to generate training examples for feature engineering. An event time series from customer transactions data base is chosen as an example. Each node represents a customer transaction and colors represent different types of events - \textit{blue- purchase}, \textit{yellow - browse}. Exact time stamps are shown below the node.  For this customers data, it sets 4 $t_c$'s. The labeling window is set as 1 event and the outcome of interest is \textit{whether or not a customer makes a purchase}. In training examples are extracted based $lag =2$ events, and $lead= 0$. Finally, 2 non-overlapping training examples are selected ($gap$ in this case is set to zero).}
    \label{fig:label_segment}
\end{figure*}
\item \textbf{Lag}: Next, we must decide how much historical data we wish to use to predict the label. This value is known as the \textit{lag}. Numerous considerations are taken into account to pick this value, including memory and computational constraints, storage, and the amount of time that has passed since the last important event. We also pick a point to calculate the lag relative to called the \textit{anchor}. Typically, there are three options for setting the anchor: the first time or data point for the entity-instance $t_s$, the point in time $t_c - lead$, or a fixed time point in the entity-instance's lifespan.

\item \textbf{Units}: For both \textit{lead} and \textit{lag}, we specify the amount of past data in absolute units- seconds. We allow users to specify in relative units-the last 10 samples or events. When relative units are specified a function transforms them into time delta in seconds by scanning the data. 

\end{itemize}



\noindent \textbf{Considerations for selecting from labeled examples}: After the label step, a given entity-instance may lead to multiple occurrences of the outcome of interest. For example, a customer may have bought a particular product multiple times, or a patient may have several seizure events. In such cases, the user must decide whether to extract multiple training examples, and, if they choose to extract just one, which one they should pick. Below, we walk through these choices, and the considerations they entail. 
\begin{itemize}
    \item {Picking multiple examples}: The user may choose to extract training examples (and their corresponding learning segments) from a single entity-instance's data. In cases where not many instances of the entity exist, this is a valuable way to maximize training examples. In particular, the user may wish to extract non-overlapping learning segments using the \textit{gap} parameter. Two learning segments are considered non-overlapping when the segments between their $t_{start}$ and $t_{stop}$ points do not overlap. In order to extract multiple exemplars, the segmentation algorithm must iterate over the labeled examples to find non-overlapping segments where the $gap$ constraint is satisfied. In algorithm~\ref{segment}, we present a greedy approach to extracting non-overlapping learning segments.   
    \item {Picking a single example}: When the user chooses to create only one example from each entity-instance, a natural question is: which one? Two possible choices are:
    \begin{itemize}
        \item First: the user may choose the first occurrence. 
        \item Random: the user may pick an example randomly. \footnote{This allows a possible feature that counts the number of past occurrences of an outcome, which could be predictive of the outcome in future.} 
    \end{itemize}
    \item {Maintaining class balance}: When there are multiple examples from the same entity instance, both positive and negative, we choose those that help maintain the balance.  
\end{itemize}
\vspace{-2mm}
\noindent \textbf{Segmentation algorithm}: With \textit{lead} and \textit{lag} defined, and either single or multiple training examples chosen, we present a greedy approach to form \ls in Algorithm \ref{segment}. It is important to note that the segmentation algorithm does not use any information from the \anns or the traversal algorithm other then the list of labeled exemplars. Unlike traversal algorithm, it does not operate on the actual data. Similar to the traversal algorithm, we see different ways to design the segmentation algorithm. 

%\input{FormSegment}

%\subsection{User interaction}

%For a given dataset D, a user will define the following to interact with the prediction engineering framework: 
%\begin{itemize}
    %\item an outcome function $ <t_c, e_{id}, l> \leftarrow O(e_{id})$.
   % \item the $lag$, which determines the amount of history to use.
    %\item the prediction window $t+l \dots T$, denoting the time over which the prediction is made.
    % \item the $lead$, indicating how far ahead we want to predict.
  %  \item And optionally other parameters: \textit{anchor}, \textit{gap}, \textit{multi}, \textit{randomize}. 
%\end{itemize} 


==> misc.tex <==


%To study how data scientists and domain experts interact, we designed a web interface with two primary modes of interaction

%\begin{enumerate}
  %\item Creating predictive models
  %\item Judging predictive models
%\end{enumerate}

 

%\subsection{Creating Predictive Models}

%For data scientists creating predictive models our interface provides three key steps where users can provide input
  %  
   % \begin{enumerate}
   %   \item Prediction Problem Definition
  %    \item Machine Learning Optimization
  %    \item Modeling report Submission
  %  \end{enumerate}
    
%Behind the scenes, Prediction Factory automates finding training examples and feature engineering.

==> pred_eng.tex <==
\section{Prediction Engineering}\label{pred_eng}
A crucial step in a successful predictive modeling project is defining how to map a business need to a technical prediction problem. We call this process``Prediction Engineering''. Today, it is done in an adhoc manner across datasets, organizations, and domains. However, as we work through numerous data science problems across domains, we identified several underlying commonalities. 

In a typical situation, a data scientist building a predictive model will start by working with a written or spoken definition of the \oc the end user is interested in predicting, as well as constraints, such as how far ahead of time the end user wishes to make the prediction (\textit{lead}) or how much data should be used to do so \textit{lag}. Given this information, we divide the workflow, in which raw data is transformed into training examples, into two steps: \textit{Label}, \textit{Segment}. 

\begin{itemize}
    \item [--] \textbf{Label}: Programmatically defining an outcome (often called label) to predict, and implementing a procedure to identify historical occurrences of the outcome. 
    \item [--] \textbf{Segment}: extracting data relevant for prediction
\end{itemize}


In the next two subsections, we describe our formalization of these two steps and how they enable  generation of outcome functions and automatic creation of training examples that we will use in Prediction factory. 

\noindent \textbf{Label}: The goal of the Label step is to traverse through an entity-instance's data and identify a list of three tuples: $< eid, t_c, l>$, where $eid$ identifies the entity-instance to which the training example belongs, $t_c$ the \co time point (or index) prior to which data can be used for learning the model, and $l$ the category of outcome (in binary cases, "positive" or "negative"). We further break this step down into two substeps: 
\begin{enumerate}
   \itemsep-0.1em
\item defining a \ann and 
  \item traversing the data in search of labels.
\end{enumerate}

\noindent \textbf{Defining a \ann:} A \ann, $L(.)$, contains a user-defined logic that
\begin{itemize}
 \itemsep-0.1em
\item is applied to the the data within the \lw,
\item can optionally use data prior to the \co $t_c$, but must use the data within the \lw, and
  \item produces a \textit{label} the user is interested in predicting.
\end{itemize}
 \begin{figure}%{r}{0.25\textwidth}
\centering
\includegraphics[width=0.85\linewidth]{Figures/FeatureReduce.pdf}
\caption{The \textit{feature-reduce} abstraction for defining prediction labels. It works by calculating a feature value for each event/sample in the labeling window. In this example, we are calculating a binary feature at each event (purchase event or not). Then, it reduces that list of features to a single label using a function such as \textsc{any}}
\end{figure}

Noting consistencies between label functions, we created the \textit{feature-reduce} abstraction. This abstraction allows data scientists to develop their own labeling functions with the same language they will later use to develop features.

% Examples of how \textit{feature-reduce} is applied in 3 different problems in 3 different domains can be seen in Table \ref{tab:examples}. 
% \input{table3_2}

\noindent \textbf{Traversal algorithm}: Given the \ann, our next goal is to design a traversal algorithm that searches through the data to identify several possible training examples. A simple design of such an algorithm would entail setting $t_c$ at every time point where a data sample is present in the entity-instance's time span, and evaluating the \ann.  

\input{search}

To do this in a tractable way, we propose to iterate over the data samples by specifying the number of $t_c$'s to consider, $n_w$, the spacing between them, $O$, and the size of the \lw, $w_l$. Pseudocode is presented in Algorithm \ref{search}. It is important to note that the traversal algorithm does not make use of any information about the logic inside the \ann. The only information that is shared between it and the \ann is the length of \lw. 

% MK - do we have space for this graphic?
% , and the process is illustrated through an example retail dataset in Figure \ref{fig:label_segment}


% We imagine that several different and perhaps efficient alternatives are possible for the traversal algorithm. To preserve generalizability, we recommend alternate designs to follow the abstractions for the labeling function, and the inputs and outputs, we suggest for the algorithm. For example, an alternate algorithm can use the size of \lw to skip portions of time series after one instance label is found. While using information from the logic inside the labeling function can aid in an efficient traversal, it could potentially result in a very specific traversal algorithm. 

\noindent \textbf{Segment}:
Given the \textit{lead} and \textit{lag} parameters and the labels, this step identifies segments defined by the four tuples $< eid, t_{start}, t_{stop}, l>$, where $t_{start}$ and $t_{stop}$ represent the time points that will bound the samples used for learning. We call this the ``\textit{learning segment.''} 
%Segmenting entails identifying the \ls for each training example, so they can be passed to the feature engineering step. A learning segment is defined by $t_{start}$, $t_{stop}$, $l$, and $e_{id}$. The first two points, $t_{start}$ and $t_{stop}$, identify start and stop times that define a segment of data that could be used to learn a machine learning model (via. feature engineering and modeling). A segmenting algorithm receives the list of all possible training examples from the \textit{annotation} phase. Next present multiple considerations that determine of how segment and subselect from the annotation examples.



% \input{segment}
\noindent \textbf{Lead, Lag, and units} 
\begin{itemize}
\item \textbf{Lead}: For a predictive problem, the $lead$ time specifies how far ahead the user wants to predict the label. For many predictive problems, predicting far ahead (high $lead$) enables value creation, and makes predictive problems interesting. For example, a retailer may want to predict future customer churn as soon as possible. 

\item \textbf{Lag}: Next, we must decide how much historical data we wish to use to predict the label. This value is known as the \textit{lag}. Numerous considerations are taken into account to pick this value, including memory and computational constraints, storage, and the amount of time that has passed since the last important event. We also pick a point to calculate the lag relative to called the \textit{anchor}. Typically, there are three options for setting the anchor: the first time or data point for the entity-instance $t_s$, the point in time $t_c - lead$, or a fixed time point in the entity-instance's lifespan.

\item \textbf{Units}: For both \textit{lead} and \textit{lag}, we specify the amount of past data in absolute units- seconds. We allow users to specify in relative units-the last 10 samples or events. When relative units are specified a function transforms them into a time delta in seconds by scanning the data. 

\end{itemize}


%\noindent \textbf{Considerations for selecting from labeled examples}: After the label step, a given entity-instance may lead to multiple occurrences of the outcome of interest. For example, a customer may have bought a particular product multiple times, or a patient may have several seizure events. In such cases, the user must decide which label to pick. Below, we walk through these choices

%\begin{itemize}
    %\item {Picking multiple examples}: The user may choose to extract training examples (and their corresponding learning segments) from a single entity-instance's data. In cases where not many instances of the entity exist, this is a valuable way to maximize training examples. In particular, the user may wish to extract non-overlapping learning segments using the \textit{gap} parameter. Two learning segments are considered non-overlapping when the segments between their $t_{start}$ and $t_{stop}$ points do not overlap. 
    
    % In order to extract multiple exemplars, the segmentation algorithm must iterate over the labeled examples to find non-overlapping segments where the $gap$ constraint is satisfied. In algorithm~\ref{segment}, we present a greedy approach to extracting non-overlapping learning segments.   
    %\item {Picking a single example}: When the user chooses to create only one example from each entity-instance, a natural question is: which one? Two possible choices are:
    %\begin{itemize}
      %  \item First: the user may choose the first occurrence. 
     %   \item Random: the user may pick an example randomly. \footnote{This allows a possible feature that counts the number of past occurrences of an outcome, which could be predictive of the outcome in future.} 
   % \end{itemize}
   % \item {Maintaining class balance}: When there are multiple examples from the same entity instance, both positive and negative, we choose those that help maintain the balance. 
%\end{itemize}

\vspace{-2mm}

With \textit{lead} and \textit{lag} defined, we use a greedy approach to form multiple \lw.

By formalizing and generalizing the process of fully specifying a prediction problem, and creating training examples, we can address a diverse set of problems in one framework. This enables us to automate the process of specifying the prediction problems by defining options for labeling function and then subsequently labeling and segmenting the data. To do this, user can simple create options for the following:
\begin{itemize}
\item[--] Entity for which prediction is sought. 
\item[--] Field over which labeling function will be applied. 
\item[--] Feature and reduce functions. 
\item[--] Labeling window size. 
\item[--] Lead and Lag.
\end{itemize}


It further allows to rapidly find training examples for a wide range of problems automatically. 
With Prediction Engineering, data scientists can easily go from a prediction problem definition to data that is ready for machine learning. 


% \begin{figure*}[htb!]
%     \centering
%     \includegraphics[width=0.9\textwidth]{figures/label_segment}
%     \caption{Figure illustrating the process of traversing, labeling, and segmenting the data to generate training examples for feature engineering. An event time series from customer transactions data base is chosen as an example. Each node represents a customer transaction and colors represent different types of events - \textit{blue- purchase}, \textit{yellow - browse}. Exact time stamps are shown below the node.  For this customers data, it sets 4 $t_c$'s. The labeling window is set as 1 event and the outcome of interest is \textit{whether or not a customer makes a purchase}. In training examples are extracted based $lag =2$ events, and $lead= 0$. Finally, 2 non-overlapping training examples are selected ($gap$ in this case is set to zero).}
%     \label{fig:label_segment}
% \end{figure*}

==> search.tex <==
\begin{algorithm}
\caption{Traversal algorithm}\label{search}
\begin{algorithmic}[1]
\Procedure{Traverse}{$L(.)$,$O$, $w_l$, $n_w$, $eid^D$, $eid$, $A$}
\State $eid^D$: Data from an entity instance $eid$. 
\State $t_s \gets starttime(eid)$ 
\State $T_c \gets $ \textsc{Set-cutoff-times} $(O, t_s, n_w)$
\For{$t_c \in T_c$}
  \State $D \gets eid^D [t_s : t_c+w_l]$ \\
  \State $l \gets L(D)$
  \State $A \cup $ \{ $eid$, $t_c$, $l$ \}
\EndFor
\State \Return $A$
\EndProcedure
\\
\Procedure{set-cutoff-times}{$O$, $t_s$, $n_w$}
\State $T_c [1] = t_s$
\For{$i = 2$ to $n_w$}
  \State $T_c [i] = (T_c[i-1] + O)$
\EndFor
\State \Return \{ $T_c$ \}
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> segment.tex <==
\begin{algorithm}
\caption{Segmentation algorithm}\label{segment}
\begin{algorithmic}[1]
\Procedure{Segment}{A, \textit{lag}, \textit{lead}, \textit{anchor}, \textit{gap}, \textit{multi}, \textit{randomize}}
\State S=\{ \}
\For{$id \in eid$}
  \State $t_s \gets starttime(id)$
  \State $T \gets {t_c}$ \emph{where}  $eid=id$ \emph{and} $ t_c > t_s+lead+lag$
  \State $ \bar l \gets {l}$ \emph{where}  $eid=id$ \emph{and} $ t_c > t_s+lead+lag$
  \If{\textit{anchor} $=$ '\textsc{start}'}
      %\State $t \gets T [1]$
      \State $t_{stop}=t_s + lag$
      %\If{$t_{stop} < t$}
         \State \Return $S \cup $$\{eid, t_s, t_{stop}, \bar l[1]\}$
       %\Else \Return \{ \}
       %\EndIf
  \ElsIf{\textit{multi} $=$ `\textsc{False}'}
         \If{\textit{randomize} $=$ `\textsc{true}'}
             \State $index \gets rand(len(T))$
             \State $t \gets T [index] $
             \State $l \gets \bar l[index] $
             \State $S \cup $ \textsc{FormSegment}($eid$, $t$, $lead$, $lag$, $l$)
         \ElsIf{\textit{randomize} $=$ `\textsc{false}'}
             \State $t \gets T [1] $
             \State $l \gets \bar l[1] $
             \State $S \cup $ \textsc{FormSegment}($eid$, $t$, $lead$, $lag$, $l$)
         \EndIf
    \ElsIf{\textit{multi} $=$ '\textsc{true}'}
          \State $q \gets t_s + lead + lag$ 
          \For{$t \in T$}
              \If{$t >q$}
                  \State $index \gets \textsc{find}(T==t)$
                  \State $l \gets \bar l [index]$
                  \State $S \cup $ \textsc{FormSegment}($eid$,$t$, $lead$, $lag$, $l$)
                  \State $q \gets t+ gap + lag +lead$
               \Else { }  $S \cup $ \{ \}
              \EndIf
          \EndFor
    \EndIf
\EndFor
\EndProcedure
\\
\Procedure{FormSegment}{$eid$, $t$, \textit{lead}, \textit{lag}, $l$}
%\State $q= t_s+ lead + lag $
%\If{$t>q$}
   \State $t_{stop} \gets {t}-lead$
   \State $t_{start} \gets t_{stop}-lag$
   \State \Return $\{eid, t_{start}, t_{stop}, l\}$
 %\Else
    %\State \Return \{ \}
%\EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}


==> survey.tex <==


Each participant filled out a brief survey asking the following multiple choice questions:

\begin{enumerate}
    \item What is the primary focus of your current job? 
\\
\begin{itemize}
            \item Data Science
            \item Product
            \item Software Engineering
            \item Analytics
            \item Management
            \item Executive
            \item Other
    \end{itemize}
    \item Does your job involve developing or using predictive models?
\\
\begin{itemize}
             \item Yes, day to day
             \item Yes, occasionally
             \item Yes, but infrequently
             \item No
    \end{itemize}
\item How many years of experience do you have working with data?
\\
 \begin{itemize}
              \item 0-1
              \item 1-3
              \item 3-5
              \item 5+'
    \end{itemize}
\item What is the main challenge you face when applying data science to business problems?
\\
\begin{itemize}
       \item Lack of talent
       \item Availablility of data
       \item Requires too much investment
       \item Defining a use case
       \item Data preparation and cleaning
       \item Other
    \end{itemize}
\end{enumerate}








==> temp.tex <==




